Simulation of positive streamers in CO$_2$ and in air: the role of photoionization or other electron sources

Positive streamer discharges have been studied and modelled extensively in air. Here we study positive streamers in CO$_2$ with and without oxygen admixtures; they are relevant for current high voltage technology as well as for discharges in the atmosphere of Venus. We discuss that no efficient photoionization mechanism is known for gases with a large CO$_2$ fraction, as photons in the relevant energy range are rapidly absorbed. Hence positive streamers can propagate only due to some other source of free electrons ahead of the ionization front. Therefore we study positive streamer propagation in CO$_2$ with different levels of background ionization to provide these free electrons. The effect of replacing photoionization by background ionization is studied with simulations in air. Simulating streamers in background fields of 16 to 20~kV/cm at standard temperature and pressure within a gap of 6.4~cm, we find that streamer propagation is rather insensitive to the level of photoionization or background ionization. We also discuss that the results depend not only on the value of breakdown field and applied electric field, and on preionization or photoionization, but also on the electron mobility $\mu(E)$ and the effective ionization coefficient $\alpha_{\rm eff}(E)$, that are gas-dependent functions of the electron energy or the electric field.

==> CO2streamers.tex <==
\section{Streamers in CO$_2$:N$_2$:O$_2$ mixtures}

\label{sec:different-gases}
\begin{figure}
  \begin{center}
    \includegraphics[width=1.1\linewidth]{CO2/figure_for_paper/diff-gas-E.pdf}
    \caption{The electric field profile for the four gas mixtures at similar streamer length and therefore different times. The background electric field is $E=16$~kV/cm~(top) and $E=0.6~E_{\rm br}$~(bottom), where $E=E_{\rm br}$ is the breakdown field, which is indicated in figure~\ref{fig:drift-diffusion-coeff-all} for each gas.
    The simulation domain extends up to 16~mm in the radial direction, but only 5~mm is shown.
    }
    \label{fig:electric-field-25ns}
  \end{center}
\end{figure}

\begin{figure}
  \begin{center}
    %\includegraphics[width=0.95\linewidth]{CO2/streamer_length-16.png}
     \includegraphics[width=0.95\linewidth]{CO2/velocity-16.png}
    \includegraphics[width=0.95\linewidth]{CO2/Emax-16.png}
     \includegraphics[width=0.95\linewidth]{CO2/radius-16.png}
    \caption{From top to bottom: streamer velocity, maximal electric field, and radius for different gas mixtures. The background electric field is 16~kV/cm.}
    \label{fig:E-L-v-1}
  \end{center}
\end{figure}

\begin{figure}
  \begin{center}
 %   \includegraphics[width=\linewidth]{CO2/axial/axial-CO2_37.png}
     \includegraphics[width=\linewidth]{CO2/axial/axial-CO2_2cm_modified.pdf}
    \caption{The electron density~(top) and the electric field~(bottom) on the symmetry axis at similar streamer length~(different times, as indicated in figure~\ref{fig:electric-field-25ns}) for different gas mixtures. The background electric field is 16~kV/cm.}
    \label{fig:axial-30}
  \end{center}
\end{figure}

\subsection{Overview of results in different gas mixtures}
\label{sec:overv-results-diff}

In this section our aim is to characterize streamer properties in the four gas mixtures that are listed in table~\ref{tbl:gases}.
% Jannis removed: Our motivation for such selection is described in the introduction. 
%Streamer discharges in air have been studied extensively, therefore they provide a good reference for streamer properties in other gases. SHARPER REFERENCE OR REMOVE REPETITION: In the introduction, we explained that often CO$_2$ is mixed with O$_2$ or N$_2$ or both in most practical applications. Furthermore, the gases that are used in experiments always contain a certain level of impurities. Therefore, here we include either a $10\%$ or a $1\%$ admixture of air into CO$_2$, and we simulate positive streamers in these mixtures that we gave the nicknames CO$_2^{(0.1)}$ and CO$_2^{(0.01)}$ in table~\ref{tbl:gases}.
%
%REFER TO EARLIER TABLE/DISCUSSION AND USE ITS NOTATION HERE:
As discussed in section~\ref{sec:review}, in CO$_2^{(0.1)}$ and CO$_2^{(0.01)}$, the photo-ionization of the air admixture is dominant. The photon absorption length in CO$_2^{(0.1)}$ is ten times longer than in air. This may affect the streamer properties. To distinguish the influence of the photon absorption length from changes in the transport and reaction coefficients, we also model positive streamers in N$_2^{(0.1)}$, which has a similar photon absorption length as CO$_2^{(0.1)}$~(see table~\ref{tbl:gases}). By comparing positive streamers in CO$_2^{(0.1)}$, N$_2^{(0.1)}$, and air we can therefore better understand why differences arise. The delayed photo-ionization model is used (see section~\ref{sec:photoi-model}), but we remark that the delay has no significant effect on the results presented here.

% One should note that using the instantaneous photo-ionization model does not change the results. {\bf Behnaz: maybe removing the last sentence?} Jannis: indeed.
Figure~\ref{fig:electric-field-25ns} shows the electric field profile of the streamers in the four gas mixtures, where in the top row of panels a homogeneous electric field of 16~kV/cm is applied while at the bottom row the electric field is $0.6E_{\rm br}$. $E_{\rm br}$ is the breakdown field, which for each gas is indicated in figure~\ref{fig:drift-diffusion-coeff-all}. \hl{Jannis: also mention kV/cm for this case? Perhaps in the figure.} To see the differences between the streamers in the four gas mixtures more clearly, the electric field profiles are shown at the same streamer length, but at different times, as indicated. It is clearly visible that the streamer is wider in CO$_2^{(0.1)}$ and CO$_2^{(0.01)}$.

% Jannis: I have removed this text
% Initially, charge separation occurs in the initial seed, which enhances the electric field and thereby starts the streamer growth. In this paper, we focus on propagation of the streamer away from the initial seed~(which depends on the initial conditions) and away from the top boundary.

%
%DISTINGUISH BETTER BETWEEN INITIAL TRANSIENTS THAT DEPEND ON THE INITIAL CONDITIONS,
%AND THE LATER EVOLUTION THAT WE WANT TO FOCUS ON.
Figure~\ref{fig:E-L-v-1} shows a more quantitative analysis of the streamer velocity, maximal electric field, and radius for $E=16$~kV/cm. The following observations can be made:\\
\textbf{Velocity} The streamer in CO$_2^{(0.1)}$ propagates with the
highest velocity. The streamer in CO$_2^{(0.01)}$ is slower than in
CO$_2^{(0.1)}$, but faster than in air, and the streamer in N$_2^{(0.1)}$ is
the slowest.\\
\textbf{Maximal electric field} In all cases, the maximal electric field
shows an initial enhancement until the positive streamer starts to propagate.
The maximal electric field of CO$_2^{(0.01)}$ is around 10~kV/cm higher than
in air. During the propagation phase, the maximal field in CO$_2^{(0.1)}$ and
N$_2^{(0.1)}$ is lower than in air.\\
\textbf{Radius} The streamer radius versus length shows two groups: in
CO$_2^{(0.1)}$ and CO$_2^{(0.01)}$ the radius is about twice that of air and
N$_2^{(0.1)}$.

In figure~\ref{fig:axial-30} the electron density~(top) and the electric field~(bottom) on the axis at different times~(as indicated in figure~\ref{fig:electric-field-25ns}) are plotted. The behavior in the region $0<z<0.5$~cm is due to the initial conditions, which we do not focus on here. The electric field in the streamer interior is slightly below 5~kV/cm for CO$_2^{(0.1)}$ and CO$_2^{(0.01)}$, whereas for air and N$_2^{(0.1)}$ is around 10~kV/cm. In addition, the value of electron density on the axis for CO$_2^{(0.1)}$ is a little higher than in air.    

%DISSTINGUISH BETWEEN DIFFERENT ZONES OF THE STREAMER IN THE DISCUSSION.

Because streamer discharges are strongly non-linear phenomena, it is not
directly clear what causes the differences between the four gas mixtures. To
address this question, we first look at the effect of transport and reaction
parameters in section~\ref{sec:impact-transp-react}. Afterwards, we discuss the
effect of photo-ionization in section \ref{sec:impact-photo-ioniz}.

\subsection{The impact of transport and reaction parameters}
\label{sec:impact-transp-react}

\hl{Jannis: it is not fully clear to me what is used for photoionization in this
  section.}

To determine the impact of the transport coefficients~($\mu_e$, $D_e$ and
$\alpha_{\rm eff}$) on streamer properties, we have performed simulations in air
where we changed one of the aforementioned parameters with that of pure CO$_2$.
\hl{Note that changing the mobility also changes the ionization source term in
  equation} (\ref{eq:dt-ne}), since
$S_i - S_\mathrm{attach} = \alpha_{\rm eff} n_e \mu_e|\bf{E}|$. All simulations were performed in a background field of $16 \, \textrm{kV/cm}$.

As expected, the diffusion coefficient $D_e$ was found to play a minor role in
the streamer properties compared to the electron mobility $\mu_e$ and the
effective ionization coefficient $\alpha_{\rm eff}$. Figure~\ref{fig:E-L-v-2}
shows the streamer velocity, maximal electric field, and radius for
cases in which $\mu_e$ and $\alpha_{\rm eff}$ were changed. Electron density and electric field profiles on the symmetry axis are compared in figure~\ref{fig:axial-2},
for streamers of the same length~(so at different times).

The streamer velocity and radius show similar behavior when the transport
coefficients are changed. In CO$_2$, streamers are faster and have a larger
radius than in air. The results for air with the mobility or the ionization
coefficient of CO$_2$ lie approximately in between these two cases, indicating
that each transport coefficient contributes about half of the observed
difference.

The maximal electric field is slightly higher in air than in CO$_2$. Using the
mobility of CO$_2$ has only a small effect, but using the ionization coefficient
of CO$_2$ significantly reduces the maximal field. For the interior electric
field shown in figure \ref{fig:axial-2}, the significance of these parameters is
reversed. With the mobility of CO$_2$, the interior field is reduced from
10~kV/cm to 5~kV/cm, whereas using the ionization coefficient of CO$_2$ has only
a small effect. The electron density in the channel is similar for the different gases, but it is slightly higher for a streamer in CO$_2$.

\begin{figure}
  \begin{center}
    %\includegraphics[width=0.95\linewidth]{air-with-CO2parameters/streamer_length.png}
    \includegraphics[width=0.95\linewidth]{air-with-CO2parameters/velocity.png}
    \includegraphics[width=0.95\linewidth]{air-with-CO2parameters/Emax.png}
    \includegraphics[width=.95\linewidth]{air-with-CO2parameters/radius.png}
    \caption{From top to bottom: maximal electric field, velocity, and radius. The background electric field is $E=16$~kV/cm.}
    \label{fig:E-L-v-2}
  \end{center}
\end{figure}

\begin{figure}
  \begin{center}
 \includegraphics[width=\linewidth]{air-with-CO2parameters/axial_2cm_modified.pdf}
    \caption{The electron density~(top) and the electric field~(bottom) on the symmetry axis at similar streamer length. The background electric field is 16~kV/cm.}
    \label{fig:axial-2}
  \end{center}
\end{figure}

\subsubsection{What causes a larger radius in CO$_2$?}

Since the streamer's velocity, radius and maximal electric field are all closely
related to each other \cite{naidis_positive_2009}, changing a transport
coefficient affects all of these properties. However, if we have to single out
one of them, it is the radius. Figures \ref{fig:electric-field-25ns},
\ref{fig:E-L-v-1} and \ref{fig:E-L-v-2} all show that streamers in CO$_2$ tend
to have a significantly larger radius than in air, under otherwise similar
conditions. As shown in figure \ref{fig:E-L-v-2}, the mobility and the
ionization coefficient each contribute about half the observed difference.

We first discuss the effect of the electron mobility. Figure
\ref{fig:drift-diffusion-coeff-all} shows that the mobility in CO$_2$ is
significantly higher than in air for fields between $3$ -- $10 \, \textrm{kV/cm}$. Figure \ref{fig:axial-2} shows that the electric field
inside the streamer channel is in this range, and that electron densities are
similar for air and CO$_2$. Streamers in CO$_2$ therefore have a higher electric
conductivity $\sigma \approx e \mu_e n_e$, which explains why they have a lower
internal electric field and thus also a lower potential drop along the channel.
A streamer in CO$_2$ therefore has a larger `potential difference' available at
its head compared to a streamer in air of the same length, which leads to a larger radius.

The interior electric field can give an estimate of the streamer stability
field, which in the experiments of Ref.~\cite{Seeger_2016} is higher for CO$_2$
than air, in contrast with our results. This difference is probably caused by
the different time scales that were considered: nanoseconds in our simulations,
and microseconds in the experiments of Ref.~\cite{Seeger_2016}.

We now discuss the effect of the ionization coefficient. Figure
\ref{fig:drift-diffusion-coeff-all} shows that CO$_2$ has a lower breakdown
field than air and that $\alpha_{\rm eff}(E)$ has a steeper slope in air. Our
hypothesis is that the radius of a streamer is controlled (to some degree) by
the ratio of forward growth versus lateral growth. Since the electric field in
the forward direction is higher than in the lateral direction, the slope of
$\alpha_{\rm eff}(E)$ has an effect on the radius: the steeper the slope, the
stronger the forward growth is compared to the lateral growth, which could
explain why streamers in CO$_2$ have a larger radius.

\hl{Jannis: not sure if we should comment on $\alpha$ being larger in CO$_2$, I don't do it now because I can't easily link it to the radius}
% Furthermore, note that the effective impact ionization in CO$_2$ is slightly
% higher than in air.

\subsubsection{The mobility and the interior field}

\hl{Jannis: Why not show results for a horizontal shift in the mobility? This just changes the amplitude, which has little effect. As it is now, I would rather omit this part.}

To investigate further whether the overall shape of the mobility reduces the field inside the streamer channel or its value, specially in $3~-~10$~kV/cm range; we artificially created three mobility profiles, see figure~\ref{fig:mobility-2}. We performed three simulations in air, in which we used one of these artificial mobility curves instead of that of air. Figure~\ref{fig:axial-3} shows the electron density and electric field on the axis for these cases. We realized that regardless of the value of the maximum, in all the three cases the electric field is reduced to 5~kV/cm.  

%One can observe that by using $\mu_{0.5\rm{CO}_2}$, oscillations appear in the electron density profile. The difference between these oscillations and the ones that we observed in figure~\ref{fig:air-photon-22ns-E-L-v} is that here the oscillations are not decaying.

% \hl{Jannis: remove first part of this paragraph}
% ~(figure~\ref{fig:drift-diffusion-coeff-all}), which results in a smaller electric field enhancement at the tip of the streamer in CO$_2$. Due to the peculiar CO$_2$ mobility curve, the electric field inside the streamer channel is smaller than in air.


%\begin{figure}
%  \begin{center}
%    \includegraphics[width=0.9\linewidth]{CO2-with-airparameters/streamer_length.png}
%    \includegraphics[width=0.9\linewidth]{CO2-with-airparameters/velocity.png}
%    \includegraphics[width=0.9\linewidth]{CO2-with-airparameters/Emax.png}
%     \includegraphics[width=.9\linewidth]{CO2-with-airparameters/radius.png}
%    \caption{From top to bottm: $L(t)$, maximal electric field, velocity, and radius.}
%    \label{fig:E-L-v}
%  \end{center}
%\end{figure}

\begin{figure}
  \begin{center}
 \includegraphics[width=\linewidth]{mobility-co2-2.png}
    \caption{The electron mobility of CO$_2$, CO$_2^{(0.1)}$, and air. The artificial mobility curves are created based on the mobility of CO$_2$.}
    \label{fig:mobility-2}
  \end{center}
\end{figure}


\begin{figure}
  \begin{center}
 \includegraphics[width=\linewidth]{air-with-CO2parameters/axial_mobility_2cm_modified.pdf}
    \caption{The electron density~(top) and the electric field~(bottom) on the symmetry axis at similar streamer length. The background electric field is 16~kV/cm.}
    \label{fig:axial-3}
  \end{center}
\end{figure}

%\begin{figure}
%  \begin{center}
% \includegraphics[width=\linewidth]{air-with-CO2parameters/axial_eta_2cm.png}
%    \caption{The electron density~(top) and the electric field~(bottom) on the symmetry axis. The background electric field is 16~kV/cm.}
%    \label{fig:axial}
%  \end{center}
%\end{figure}

\subsection{The impact of photo-ionization}
\label{sec:impact-photo-ioniz}
\hl{Jannis: I've edited/simplified this a bit}

For the gas mixtures considered here, estimates for the number of emitted photons and the photon absorption length are provided in table~\ref{tbl:gases}.
In CO$_2^{(0.1)}$, ionizing radiation is produced by the 8$\%$ of N$_2$ molecules and therefore is roughly 10$\%$ of the production in air~(n$_{\rm air}$). On the other hand, having only 10$\%$ of the O$_2$ molecules in CO$_2^{(0.1)}$ compared to air leads to a 10 times longer absorption length for the photons. Both mechanisms reduce the amount of photo-ionization close to the streamer head in CO$_2^{(0.1)}$, since fewer photons are produced, and their absorption is spread out over a larger volume.

N$_2^{(0.1)}$ has the same absorption length as CO$_2^{(0.1)}$, but the number
of emitted photons is slightly higher than in air. Streamers in air,
N$_2^{(0.1)}$ and CO$_2^{(0.1)}$ were compared in section
\ref{sec:overv-results-diff}, using a background field of $E=16$~kV/cm. Electric
field profiles are shown in figure~\ref{fig:electric-field-25ns}, and the
maximal electric field, velocity, and radius are shown in
figure~\ref{fig:E-L-v-1}. Note that the streamer radius in N$_2^{(0.1)}$ is very
similar to the radius in air. There are larger differences in the maximal
electric field and the velocity, but overall streamers in N$_2^{(0.1)}$ and air
are quite similar. This suggests that the longer photon absorption length in
CO$_2^{(0.1)}$ does not play a dominant role in the streamer properties.

In CO$_2^{(0.01)}$, the number of photons produced is roughly a factor 100 lower than in air, and their absorption length is a factor 100 longer. Due to both effects, the number of photo-ionization events close to the discharge is significantly lower than in air. The continuum approximation for photo-ionization can therefore lose its validity, and a Monte Carlo approach with discrete photons~\cite{bagheri2019effect} is more appropriate; this is however outside the scope of the present paper.

%We also checked the validity of the continuum photo-ionization for the four gas mixtures. For this we performed the simulation in each gas with Monte Carlo photo-ionization with discrete photons. The computed average photon absorption length is around 0.475~mm in air, 4.41~mm in 98$\%$~N$_2$~-~2$\%$~O$_2$ and CO$_2^{(0.1)}$, and 15.8~mm in $99\%$~CO2~-~$1\%$~air. The photoelectron production rate is shown in figure~\ref{fig:MC-photo-ionization} at t=5~ns. It is visible that the photons in 98$\%$~N$_2$~-~2$\%$~O$_2$ and CO$_2$ gas mixtures travel a longer distance until they are absorbed by O$_2$ molecules. This leads to a dispersed photoelectron profile. In $99\%$~CO2~-~$1\%$~air, the average absorption length is longer than the computational domain and most photons are not absorbed within the domain. This may suggest that the continuum approximation for photo-ionization in $99\%$~CO2~-~$1\%$~air might loose its validity.
%
%By increasing CO$_2$ fraction the photon absorption length is increased which is in agreement with the measurements of Seguin~{\it et al}~\cite{seguin_ultraviolet_1974}. 
%
%
% In all of these simulations the streamer branches and branching is not the focus of this work. The use of continuum approximation with axisymmetric simulation is suitable to study streamer propagation~\cite{bagheri2019effect}.  

%
%\begin{figure}
%  \begin{center}
%    \includegraphics[width=\linewidth]{photoionization/drawing.pdf}
%    \caption{Monte Carlo photoionization. The production rate of photoelectrons on a logarithmic scale at t=5~ns using. The time step is around~2~ps.}
%    \label{fig:MC-photoionization}
%  \end{center}
%\end{figure}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Paper"
%%% End:


==> Computational-domain.tex <==
\subsection{Computational domain and initial conditions}
\label{sec:comp-domain}

\begin{figure}
  \centering
  {\includegraphics[width=0.3\textwidth]{Computational-domain.pdf}}
  \caption{The axisymmetric domain~($z_{\rm{max}}=3.2$~cm, and $r_{\rm{max}}=1.6$~cm) showing the position of the
    neutral seed on the axis of symmetry at $(r,z)=(0,0)$ from which the streamer starts. %The seed is about 3.84~mm long with a radius of about 0.02~mm. It has an electron and positive ion density of $5\cdot10^{19}$~$\rm{m}^{-3}$ at its center, which decays at distances above $d = 0.1$~mm with a smoothstep profile: $1-3x^2 + 2x^3$
%, where $x = (d-0.1~{\rm mm})/0.1~{\rm mm}$. 
The boundary at $z=0$~cm is at a potential $\Phi=\Phi_0$ and the boundary at $z=3.2$~cm
is grounded. For the potential, 
Neumann zero boundary conditions are used
at $r=0$~(due to symmetry), and $r=r_{\rm{max}}$. Neumann zero boundary conditions are also applied for the electron density on all
boundaries. }
  \label{fig:computational-domain}
\end{figure}

The computational domain shown in figure~\ref{fig:computational-domain} is used for axisymmetric
simulations where $z_{\rm{max}}=3.2$~cm, and $r_{\rm{max}}=1.6$~cm. 
The boundary at $z=0$~cm is at a potential $\Phi_0$ and the boundary at $z=3.2$~cm
is grounded; hence it creates a homogeneous background electric field. In this paper we employ different values for $\Phi_0$ which leads to different background electric fields which is indicated explicitly in each section.

For the potential, 
Neumann zero boundary conditions are used
at $r=0$, and $r=r_{\rm{max}}$. Neumann zero boundary conditions are also applied for the electron density on all
boundaries. We place a neutral seed of about 3.84~mm long with a radius of about 0.02~mm at the bottom boundary on the symmetry axis, $(r,z)=(0,0)$. The seed has an electron and positive ion density of $5\cdot10^{19}$~$\rm{m}^{-3}$ at the center, which decays at
distances above $d = 0.1$~mm with a smoothstep profile: $1-3x^2 + 2x^3$
, where
$x = (d-0.1~{\rm mm})/0.1~{\rm mm}$.

%A homogeneous background density of
%$n_e=n_i=10^9 \, \textnormal{m}^{-3}$ electrons and positive ions is included.
%% Furthermore, an axisymmetric domain with $r_{\mathrm{max}} = z_{\mathrm{max}} = 1.25$~cm is used in which all the other conditions are the same as above.
%For the axisymmetric simulations, we use the same computational domain as in
%\cite{bagheri_comparison_2018}.

In this paper, we use the same refinement criterion as in \cite{teunissen_simulating_2017}. The grid is refined if $\alpha(1.2 \times E) \, \Delta x > 0.8$, where $\alpha(E)$ is
the field-dependent ionization coefficient, $E$ is the electric field strength
in V/m, and $\Delta x$ is the grid spacing. This gives an AMR grid with a minimum grid spacing of
around $2 \, \mu\textrm{m}$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Paper"
%%% End:

